InstanceDiffusion: Instance-level Control for Image Generation

Text-to-image diffusion models produce high quality images but do not offer control over individual instances in the image. We introduce InstanceDiffusion that adds precise instance-level control to text-to-image diffusion models. InstanceDiffusion supports free-form language conditions per instance and allows flexible ways to specify instance locations such as simple single points, scribbles, bounding boxes or intricate instance segmentation masks, and combinations thereof. We propose three major changes to text-to-image models that enable precise instance-level control. Our UniFusion block enables instance-level conditions for text-to-image models, the ScaleU block improves image fidelity, and our Multi-instance Sampler improves generations for multiple instances. InstanceDiffusion significantly surpasses specialized state-of-the-art models for each location condition. Notably, on the COCO dataset, we outperform previous state-of-the-art by 20.4% AP$_{50}^\text{box}$ for box inputs, and 25.4% IoU for mask inputs.

==> Makefile <==
main:
	pdflatex main

full:
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main

camready: full
	gs -dNOPAUSE -dBATCH -dNOPLATFONTS -sDEVICE=pdfwrite -dEmbedAllFonts=true -sOutputFile=main-gs.pdf -f main.pdf

cut: full
	pdftk main.pdf cat 1-11 output main_submit.pdf
	pdftk main.pdf cat 12-end 9-11 output suppl_submit.pdf

clean:
	rm *.aux *.bbl *.blg *.log *.pdf *.dep *.brf *.fls *.out

run:
	evince main.pdf

compress:
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/default -dNOPAUSE -dQUIET -dBATCH -dDetectDuplicateImages -dCompressFonts=true -r150 -sOutputFile=suppl.pdf suppl_highRes.pdf

arxiv: full
	rm -rf ../arxiv.tar.gz ../paper_arXiv
	cd ../arxiv-latex-cleaner && python3.9 -m arxiv_latex_cleaner ../paper/
	# Unfortunately it still doesn't remove unused PDF etc files... need to use the arxiv-collector
	rm -f /tmp/latexmk
	cd .. && python3.9 arxiv-collector/arxiv_collector.py --get-latexmk /tmp/latexmk
	cd ../paper_arXiv && python3.9 ../arxiv-collector/arxiv_collector.py --latexmk /tmp/latexmk main.tex
	mv ../paper_arXiv/arxiv.tar.gz ../
	rm -rf ../paper_arXiv


